BehAVE: Behaviour Alignment of Video Game Encodings

Domain randomisation enhances the transferability of vision models across visually distinct domains with similar content. However, current methods heavily depend on intricate simulation engines, hampering feasibility and scalability. This paper introduces BehAVE, a video understanding framework that utilises existing commercial video games for domain randomisation without accessing their simulation engines. BehAVE taps into the visual diversity of video games for randomisation and uses textual descriptions of player actions to align videos with similar content. We evaluate BehAVE across 25 first-person shooter (FPS) games using various video and text foundation models, demonstrating its robustness in domain randomisation. BehAVE effectively aligns player behavioural patterns and achieves zero-shot transfer to multiple unseen FPS games when trained on just one game. In a more challenging scenario, BehAVE enhances the zero-shot transferability of foundation models to unseen FPS games, even when trained on a game of a different genre, with improvements of up to 22%. BehAVE is available online at https://github.com/nrasajski/BehAVE.

==> reviews.tex <==
Review 1

1. Brief summary of the paper (including a clear summary of the topic, and a justified overall recommendation)

The paper introduces a novel method for domain transferring among different videogames, based on pretrained video encodings, manually crafted semantic interpretation of base keypress sequences, and learning of a simple “translator” that puts in connection that video and text embeddings from different games. The results reported in the paper shows that the trained model achieves some reliable form of video understanding that generalizes well to different and unseen videogames, of the same and different genre. Numerical results reported in the paper seems to strongly support these claims, although other applications like imitation learning are not considered (this is clearly mentioned by the authors in the paper as a limitation / future work). This kind of work results to be fundamental for the development of game foundation models in the area of videogames and likely, in the future, even beyond this domain. I’d have appreciated some more information on the dataset and its limitation, including a clear description of its acquisition in the main text.

2. Strong points of the paper (including novelty)
The paper is well written and suitable for submission to a full conference (beyond this workshop) with some little adjustment.

Clarity is close to optimal, apart from few minor points mentioned in the next section.

The topic is definitely of interest for the community of the workshop and fundamental for the development of the current generation of foundation models working in the video game space.

Numerical results strongly support the claims done by the author.

The novelty is high – although the method is based on nowadays well established principles, i.e. mapping embeddings from different domains into a common space, their effective application to videogames is still limited, therefore I highly appreciate papers like this.

The authors also clearly discuss the limitations of their work, and help the reader understanding the important points for the development of their (and similar) models, such as the adoption of a semantic (human defined) description of keypress sequences, which is way more informative for the model with respect to raw data.

3. Weak points of the paper (highlights red flags if needed)

% Nemanja: Discussion should cover this
As clearly state by the authors as well, the method has not been designed and tested on large scale architectures and data. Given the well demonstrated capability of foundation model to greatly improve their capabilities under these circumstances, performing this kind of experiment within the already well established context of the paper could provide deep insights about the capability of foundation models to generalize to different videogames.

% Nemanja: Discussion should cover this
Another limitation, which is also clearly stated by the authors, is that the model has not been tested on imitation learning application, that could indeed be part of the next step. This limitation is understandable though, as there is clearly no space to assess all the points within the same paper with limited space available.

None of the weak points mentioned here are critical, they should rather be seen as potential improvement directions for the paper.

Another few, very minor weak points affect the paper.

% Nemanja: A very small change was added to intro
Clarity is not maximized at the beginning as I had some hard time understanding that the main scope of the paper and the experimental results mostly refer to video understanding and the analysis of the generalization capability of video understanding to different video games. I think this should be clearly stated from the very beginning of the paper.

% Nemanja: This is already explained in Section 4
Furthermore, it’s not 100\% clear what categories are considered in the video understanding set – from the tables in the paper, it looks like there are only 4 labels, which is a pretty low number. Authors should explain better this point in the main text.

4. Novelty and Innovation
The paper is somehow original

5. Experimental Validation
Experimental results supports the claims, although deeper investigation and comparison with the state of the art could make the paper stronger

6. Clarity and Presentation
The paper is clear, a minimal effort is required to reproduce the results

7. Overall recommendation
Accept

==========================================================
Review 2

1. Brief summary of the paper (including a clear summary of the topic, and a justified overall recommendation)
The paper introduces BehAVE, a novel framework designed to leverage the visual diversity inherent in commercial video games for domain randomization in video understanding tasks. The framework aligns video encoding representations based on similar player behaviors across visually distinct games that belong to the same genre (i.e., first-person shooter), without requiring access to game simulation engines. The paper proposes techniques such as Semantic Action Encoding (to translate player actions into textual descriptions) and post-training video encoding projection (to align video representation with the semantic action embeddings). The BehAVE framework is evaluated on the SMG-25 dataset, a newly introduced collection of gameplay videos from various first-person shooter (FPS) games, along with two other publicly available datasets. The clustering quality metrics are primarily used to show the improvements. The authors have done a decent job in clarity of writing, organization of the paper, and explaining the contributions. The supplementary materials provide a detailed account of the dataset collection and preprocessing, showcasing the framework’s potential in zero-shot transferability and behavior classification.

2. Strong points of the paper (including novelty)

Practical Domain Randomization Approach: The use of commercial video games for domain randomization without the need for access to game engines is a practical and innovative solution, making the framework scalable and applicable in real-world scenarios.

Comprehensive Data Collection and Preprocessing: The supplementary section offers a decent description of the data collection and preprocessing pipeline for the SMG-25 dataset, training process, and hyperparameters. The detailed methodology, including items such as label propagation and delta thresholding techniques, enhances the reliability and robustness.

Semantic Action Encoding: The use of an approach, termed semantic action encoding, to align video representations across different domains is a key innovation in this paper. It’s shown that this technique significantly improves the generalization capabilities of the framework, as demonstrated in the paper’s experiments.
Z
ero-shot Transferability and Preliminary Inverse Dynamics Modeling: The framework demonstrates (and claims) strong zero-shot transferability in behavior classification tasks, even across different game genres by presenting experiments including an out-of-domain game (Minecraft).

Potential Scalability: Despite working within a limited computational budget, the framework shows potential for scalability, particularly if extended with more data and resources. The modular nature of the data collection script also hints at broader applicability across different game genres.

3. Weak points of the paper (highlights red flags if needed)

% Nemanja: Discussion should cover this
Limited Scope of Evaluation: While the supplementary materials provide additional insights into the data collection process, the evaluation is still primarily confined to FPS games, with only preliminary exploration of cross-genre transferability. The generalizability of the findings remains limited.

% Nemanja: Discussion should also cover this
Over-reliance on Foundation Models and Lack of Fine-tuning: The framework relies heavily on pre-trained foundation models, and the supplementary section reveals that the models were not fine-tuned for the specific dataset or problem domain. This reliance may limit the framework's adaptability and performance in other domains.

% Nemanja: The metrics we used are supported by previous literature, and reviewers ask for additional ones, without saying current ones are bad, so in my opinion no need for further comments
Evaluation Metrics and Further Exploration: Although the supplementary material includes additional experimental results, the use of metrics such as silhouette scores and transferability scores may not fully capture the complexities of behavior alignment and generalization. More nuanced metrics and a deeper exploration of the framework's performance are needed. For example, experiments like low-level task performance (e.g., loading a gun) for curation and/or retraining are routinely used in similar works.

% Nemanja: Discussion should cover this
Scalability and Real-time Application Challenges: While the framework is efficient on a single GPU, the supplementary section suggests that scaling up for real-time applications or larger datasets remains a challenge. The preliminary results in inverse dynamics modeling indicate that more data and computational resources are needed for broader applicability.

% Nemanja: The paper explains the format of the dataset is (frame, actions) pairs. Player skill is not relevant to this paper. One short addition was added to section 3.2, and a small paragraph about annotators was added to supplementary material.
Need for More Dataset Details: The paper does not provide enough detail on the SMG-25 dataset, which is crucial for understanding the scope and quality of the data. Missing information includes the number of players, their skill levels, per-game state distributions, and how the one-second episodes (16 frames) are generated. These details are essential for assessing the dataset's representativeness and the reliability of the experiments.

% Nemanja: Should be covered by discussion
Use of Foundation Models: The use of foundation models in the framework appears underdeveloped. There are opportunities to enhance the capture of action semantics by incorporating more advanced models, such as Large Language Models (LLMs) and Vision-Language Models (VLMs). These could potentially provide a richer and more nuanced understanding of the actions being analyzed.

4. Novelty and Innovation
Marginally
The paper is somehow original

5. Experimental Validation
Experimental results supports the claims, although deeper investigation and comparison with the state of the art could make the paper stronger

6. Clarity and Presentation
The clarity of the paper should be improved, reproducing the results is likely possible but requires a large effort

7. Overall recommendation
Neutral

==============================================================
Review 3

1. Brief summary of the paper (including a clear summary of the topic, and a justified overall recommendation)
The paper introduces a novel framework to align player behaviors across different FPS (First-Person Shooter) games using pre-trained video and text encoders. The proposed BehAVE framework leverages the SMG-25 dataset, which comprises synchronized frames and player actions from 25 commercial FPS games. The methodology includes detailed data collection, pre-processing, and alignment processes, aiming for zero-shot transferability.

2. Strong points of the paper (including novelty)

-Novel Approach: The BehAVE framework introduces a novel method for domain randomization by utilizing existing commercial video games without accessing their simulation engines. This significantly differs from traditional methods that rely heavily on intricate simulation engines.

-Methodology: The methodology is comprehensively described, including detailed steps for data collection, pre-processing, and behavior alignment.

-Dataset: Introduction of the SMG-25 dataset, which is a valuable contribution to the field, providing a substantial amount of synchronized gameplay data across various FPS games.

3. Weak points of the paper (highlights red flags if needed)

% Nemanja: Discussion has this as future work
-Limited Scope of Experiments: The paper focuses primarily on FPS games. While it demonstrates transferability to a non-FPS game (Minecraft), further experiments across a wider range of game genres would be necessary to establish the generalizability of the approach fully.

% Nemanja: The metrics we used are supported by previous literature, and reviewers ask for additional ones, without saying current ones are bad, so in my opinion no need for further comments
-Evaluation Metrics: Using silhouette scores and transferability scores is appropriate, but additional evaluation metrics and comparisons with other state-of-the-art methods would provide a more comprehensive assessment of the framework's performance.

4. Novelty and Innovation
The paper is somehow original

5. Experimental Validation
Experimental results only partially support the claims, deeper investigation and/or comparison with state of the art are needed

6. Clarity and Presentation
The clarity of the paper is sufficient, results can be reproduced with a reasonable effort by a skilled researcher

7. Overall recommendation
Weak accept
